A Superconducting Phase Shifter and Traveling Wave Kinetic Inductance Parametric Amplifier for W-Band Astronomy

The W-Band ($75-110\; \mathrm{GHz}$) sky contains a plethora of information about star formation, galaxy evolution and the cosmic microwave background. We have designed and fabricated a dual-purpose superconducting circuit to facilitate the next generation of astronomical observations in this regime by providing proof-of-concept for both a millimeter-wave low-loss phase shifter, which can operate as an on-chip Fourier transform spectrometer (FTS) and a traveling wave kinetic inductance parametric amplifier (TKIP). Superconducting transmission lines have a propagation speed that depends on the inductance in the line which is a combination of geometric inductance and kinetic inductance in the superconductor. The kinetic inductance has a non-linear component with a characteristic current, $I_*$, and can be modulated by applying a DC current, changing the propagation speed and effective path length. Our test circuit is designed to measure the path length difference or phase shift, $\Delta \phi$, between two symmetric transmission lines when one line is biased with a DC current. To provide a measurement of $\Delta\phi$, a key parameter for optimizing a high gain W-Band TKIP, and modulate signal path length in FTS operation, our $3.6 \times 2.5\; \mathrm{cm}$ chip employs a pair of $503\; \mathrm{mm}$ long NbTiN inverted microstrip lines coupled to circular waveguide ports through radial probes. For a line of width $3\; \mathrm{\mu m}$ and film thickness $20\; \mathrm{nm}$, we predict $\Delta\phi\approx1767\; \mathrm{rad}$ at $90\; \mathrm{GHz}$ when biased at close to $I_*$. We have fabricated a prototype with $200\; \mathrm{nm}$ thick Nb film and the same line length and width. The predicted phase shift for our prototype is $\Delta\phi\approx30\; \mathrm{rad}$ at $90\; \mathrm{GHz}$ when biased at close to $I_*$ for Nb.

==> macros.tex <==
\usepackage{url}

%--- VARIOUS
\newcommand{\etal}{~et~al. }                    
\newcommand{\ojo}{\fbox{\bf !`$\odot$j$\odot$!}} 
\newcommand{\cita}{\citeasnoun}
\newcommand{\cites}{\citeaffixed}
\newcommand{\lai}{\'{\i}}
\newcommand{\y}{{\it y\ }}
\newcommand{\titlebar}{\rule{15cm}{1mm}\\[2.pt]\rule{15cm}{0.4mm}\\} 
\newcommand{\eg}{$e.g.$}

%--- UNITS
%\newcommand{\deg}{$^{\circ}}
\newcommand{\arcmin}{\hbox{$^\prime$}}               % arcmin
\newcommand{\arcsec}{\hbox{$^{\prime\prime}$}}       % arcsec
\newcommand{\kms}{ km\ s$^{-1}$}                     % km s-1
\newcommand{\ergs}{erg s$^{-1}$}                     % erg s-1
\newcommand{\ergsM}{erg s$^{-1}$Mpc$^{-3}$}          % erg s-1 Mpc-3
\newcommand{\sen}{mJy/$\sqrt{\rm Hz}$}               % Unidades de sensibilidad
\newcommand{\mic}{$\mu$m}                            % Micras!!!
\newcommand{\um}{$\mu$m}
\newcommand{\lmf}{\bf }
\newcommand{\mytilde}{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}} 
\newcommand{\HI}{\mbox{H\,\textsc{i}}}%
\def\degr   {$^\circ$}	


\newcommand{\ergseq}{{\rm erg}\: {\rm s}^{-1}\:}     % erg s-1  (eqn)
\newcommand{\Hub}{km\ s$^{-1}$ Mpc$^{-1}$}           % km s-1 Mpc-1

%Solar:
\newcommand{\Msun}{$M_{\odot}$}                       % M_o 
\newcommand{\Lsun}{$L_{\odot}$}                       % L_o 
\newcommand{\MJ}{$M_J$}                                         % M_Jup
\newcommand{\ME}{$M_{\oplus}$}                          % M_Earth
\newcommand{\Moon}{$M_{Moon}$}                          % M_Moon
\newcommand{\Planck}{{\it Planck}}   
%\newcommand{\planck}{{\it Planck}} 


\newcommand{\microns}{$\mu$m}                            % Micras!!!

\newcommand  \gtsim  {\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\newcommand  \ltsim  {\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\newcommand{\lap}{$\stackrel{<}{_\sim}$}
\newcommand{\gap}{$\stackrel{>}{_\sim}$}
\newcommand	\micron		{{\mu{\rm m}}}
%\newcommand{\arcmin}{\hbox{$^\prime$}}               % arcmin
%\newcommand{\arcsec}{\hbox{$^{\prime\prime}$}}       % arcsec


%Cosmology:
\newcommand{\Om}{$\Omega_{\rm M}$}
\newcommand{\Ol}{$\Omega_\Lambda$}
\newcommand{\Ok}{$\Omega_k$}


%----------------------- BIBTEX --------------------------
%--- JOURNALS
\newcommand{\apj}{\rm ApJ}
\newcommand{\apjl}{\rm ApJL}
\newcommand{\apjs}{\rm ApJS}
\newcommand{\aaps}{\rm A$\&$AS}
\newcommand{\aap}{\rm A$\&$A}
\newcommand{\aapr}{\rm A$\&$AR}
\newcommand{\mnras}{\rm MNRAS}
\newcommand{\aj}{\rm Astron. J.}
\newcommand{\araa}{\rm ARAA}
\newcommand{\nat}{\rm Nature}
\newcommand{\pasj}{\rm PASJ}
\newcommand{\ASP}{\rm ASP COnference Series}
\newcommand{\CASP}{\rm Comm. Astrophys. Space Phys.}
\newcommand{\astroph}{\rm astro-ph/}
\newcommand{\apss}{\rm Ap\&SS}%          % Astrophysics and Space Science
\newcommand{\qjras}{\rm QJRAS}%          % Quarterly Journal of the RAS
\newcommand{\pasp}{\rm PASP}%          % Publications of the ASP
\newcommand{\physrep}{\rm Phys. Rep.}
\newcommand{\prd}{\rm Phys. Rev. D}
\newcommand{\jcap}{\rm JCAP}% 

\def\aplett{{\it Astrophys.~Lett.}} % Astrophysics Letters
\def\ao{{\it Appl.~Opt.}}           % Applied Optics

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao


\def\K{{\rm K}}
\def\milliK{{\rm mK}}
\def\mK{{\rm \mu K}}
\def\muK{{\rm \mu K}}
\def\MJy{{\rm MJy}}
\def\Jy{{\rm Jy}}
\def\mJy{{\rm mJy}}
\def\sr{{\rm sr}}
\def\MJysr{\MJy/\sr}
\def\Mpc{{\rm Mpc}}
\def\GHz{{\rm GHz}}
\def\specint{{I_\nu}}
\def\bfzero{{\bf 0}}

\def\icm{${\rm cm}^{-1}\;$}
\def\3he{$^3{\rm He}$}
\def\arcdeg{\hbox{$^\circ$}}
\def\kusd{{K\$\phantom{0}}} %$
\def\et{{\it et al.}}
\def\COBE{{\sl COBE}}
\def\TBD{{\bf TBD}}

\def\blast{{BLAST}}
\def\blastp{{BLASTPol}}
\newcommand{\boom}{{\sl Boomerang}}
\newcommand{\wmap}{{\sl WMAP}}
\newcommand{\planck}{{\sl Planck}}
\newcommand{\spitzer}{{\sl Spitzer\/}}
\newcommand{\herschel}{{\sl Herschel}}
\newcommand{\akari}{{\sl AKARI}}
\newcommand{\hst}{{\sl HST}}
\newcommand{\chandra}{{\sl Chandra}}
\newcommand{\xmm}{{\sl XMM}}
\newcommand{\alma}{{\sl ALMA} }


%\input{aas_macros.sty}
%
% Hyphenations
%
\hyphenation{CMBR}
\hyphenation{bolo-meters}
\hyphenation{an-iso-tropy}


%--- BOOKS
\newcommand{\peacock}{\rm Cambridge University Press }
\newcommand{\avishai}{\rm Cambridge University Press }
\newcommand{\peebles}{\rm Princeton University Press }

%---------------------------------------------------------
\def\lsim{\mathrel{\lower2.5pt\vbox{\lineskip=0pt\baselineskip=0pt
           \hbox{$<$}\hbox{$\sim$}}}}

\def\gsim{\mathrel{\lower2.5pt\vbox{\lineskip=0pt\baselineskip=0pt
           \hbox{$>$}\hbox{$\sim$}}}}





